Polynomial Time Approximation Schemes for Clustering in Low Highway Dimension Graphs

We study clustering problems such as k-Median, k-Means, and Facility Location in graphs of low highway dimension, which is a graph parameter modeling transportation networks. It was previously shown that approximation schemes for these problems exist, which either run in quasi-polynomial time (assuming constant highway dimension) [Feldmann et al. SICOMP 2018] or run in FPT time (parameterized by the number of clusters $k$, the highway dimension, and the approximation factor) [Becker et al. ESA~2018, Braverman et al. 2020]. In this paper we show that a polynomial-time approximation scheme (PTAS) exists (assuming constant highway dimension). We also show that the considered problems are NP-hard on graphs of highway dimension 1.

==> preamble.tex <==
\usepackage{ifthen}
\usepackage{comment}
\makeatletter
\pdfminorversion=5


\usepackage[
style=numeric,
giveninits=true, 
maxbibnames=99, 
maxcitenames=2, 
natbib=true, 
labelnumber, 
defernumbers=true,  
backend=biber, 
sortcites=true,
doi=false,isbn=false,url=false
]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}
}
\let\oldcitet\citet
\renewcommand{\citet}[1]{\mbox{\oldcitet{#1}}}

%
%
\usepackage[margin=1in]{geometry}
\let\oldep\everypar  \newtoks\everypar  \oldep{\the\everypar\looseness=-1}
%
%
%
%

\usepackage[colorlinks=true,bookmarks=false]{hyperref}
\usepackage[small,bf]{caption}
%
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[british]{babel}
\usepackage{paralist}
\usepackage[shortlabels]{enumitem}
\setlist[enumerate]{nosep} %
\setlist[itemize]{nosep} %

\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.45}
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0.13,0.5,0}
\hypersetup{colorlinks, linkcolor=darkblue, citecolor=darkgreen,
urlcolor=darkblue}

\usepackage{amsthm}


\usepackage{amsmath,amsfonts,amssymb}
\usepackage{mathtools}
\usepackage{mathrsfs}
%
\usepackage{floatflt}
\usepackage{floatrow} %
\usepackage{xspace}
\usepackage{csquotes}
\usepackage{multirow}

%
%

%

\usepackage[nameinlink,capitalise]{cleveref}

\usepackage{footmisc}

\usepackage{aliascnt}
\newtheorem{theorem}{Theorem}%
\newaliascnt{lemma}{theorem}
\newaliascnt{corollary}{theorem}
\newaliascnt{definition}{theorem}
\newaliascnt{claim}{theorem}
\newaliascnt{prop}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\newtheorem{claim}[claim]{Claim}
\newtheorem{corollary}[corollary]{Corollary}
\newtheorem{prop}[prop]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{lemma}
\aliascntresetthe{corollary}
\aliascntresetthe{definition}
\aliascntresetthe{claim}
\aliascntresetthe{prop}

%
%
%
%
%
%
%
%


%
\newcommand{\ol}[1]{{\overline{#1}}}
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\cqed}{\renewcommand{\qed}{\hfill$\lrcorner$}}

%

%
\newcommand{\hy}{\hbox{-}\nobreak\hskip0pt}

%
%

%
%
\usepackage{environ,xstring}
\newif\iflabel
\newif\ifdbs
\newif\ifamp
\NewEnviron{doitall}{%
  \noexpandarg
  \expandafter\IfSubStr\expandafter{\BODY}{\label}{\labeltrue}{\labelfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{\\}{\dbstrue}{\dbsfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{&}{\amptrue}{\ampfalse}%
  \iflabel\def\doitallstar{}\else\def\doitallstar{*}\fi
  \ifdbs
    \ifamp
      \def\doitallname{align}%
    \else
      \def\doitallname{multline}%
    \fi
  \else
    \def\doitallname{equation}
  \fi
  \begingroup\edef\x{\endgroup
    \noexpand\begin{\doitallname\doitallstar}%
    \noexpand\BODY
    \noexpand\end{\doitallname\doitallstar}%
  }\x
}
\def\[#1\]{\begin{doitall}#1\end{doitall}}

\newcommand{\pname}[1]{\textsc{#1}}
\newcommand{\todo}[1]{\textcolor{red}{$\ll$\textsf{TODO: #1}$\gg$}}
\newcommand{\aef}[1]{\textcolor{red}{$\ll$\textsf{Andreas: #1}$\gg$}}
\newcommand{\david}[1]{\textcolor{red}{$\ll$\textsf{David: #1}$\gg$}}

\usepackage{thm-restate}

\usepackage{framed}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


